DistrictNet: Decision-aware learning for geographical districting

Districting is a complex combinatorial problem that consists in partitioning a geographical area into small districts. In logistics, it is a major strategic decision determining operating costs for several years. Solving districting problems using traditional methods is intractable even for small geographical areas and existing heuristics often provide sub-optimal results. We present a structured learning approach to find high-quality solutions to real-world districting problems in a few minutes. It is based on integrating a combinatorial optimization layer, the capacitated minimum spanning tree problem, into a graph neural network architecture. To train this pipeline in a decision-aware fashion, we show how to construct target solutions embedded in a suitable space and learn from target solutions. Experiments show that our approach outperforms existing methods as it can significantly reduce costs on real-world cities.

==> algorithms/perturbation.tex <==
\begin{algorithm}[htb]
    \caption{Perturbation for Districting}
    \label{alg:perturbationDistricting}
    \begin{algorithmic}
        \REQUIRE Current districting solution $S$
        \ENSURE Perturbed solution

        \FOR{each pair of districts $(D_i, D_j)$ in random order}
            \STATE Identify border nodes between $D_i$ and $D_j$
            \FOR{each border node $\text{node}_i$ in $D_i$ and $\text{node}_j$ in $D_j$}
                \STATE With a certain probability, apply perturbation: relocate $\text{node}_i$ to $D_j$ or swap $\text{node}_i$ with $\text{node}_j$
            \ENDFOR
        \ENDFOR
    \end{algorithmic}
\end{algorithm}
